Are Larger Pretrained Language Models Uniformly Better? Comparing Performance at the Instance Level

Larger language models have higher accuracy on average, but are they better on every single instance (datapoint)? Some work suggests larger models have higher out-of-distribution robustness, while other work suggests they have lower accuracy on rare subgroups. To understand these differences, we investigate these models at the level of individual instances. However, one major challenge is that individual predictions are highly sensitive to noise in the randomness in training. We develop statistically rigorous methods to address this, and after accounting for pretraining and finetuning noise, we find that our BERT-Large is worse than BERT-Mini on at least 1-4% of instances across MNLI, SST-2, and QQP, compared to the overall accuracy improvement of 2-10%. We also find that finetuning noise increases with model size and that instance-level accuracy has momentum: improvement from BERT-Mini to BERT-Medium correlates with improvement from BERT-Medium to BERT-Large. Our findings suggest that instance-level predictions provide a rich source of information; we therefore, recommend that researchers supplement model weights with model predictions.

==> Instance-level/0124_improvement_hist.tex <==
\section{Instance Difference} \label{sec:main-comparison-2models}


























\iffalse
Since model predictions vary across random seeds, we cannot claim that certain model size $s$ predicts an instance $i$ completely (in)correctly.
Instead, we define the \textit{instance accuracy} $\acc^{s}_{i} \in [0, 1]$:
\begin{equation}
    \acc_{i}^{s} := \mathbb{E}_{P,F}[c^{i,s}].
\end{equation}
i.e. how often model of size $s$ predicts instance $i$ correctly.
When we compare two model sizes $s_{1}$ and $s_{2}$, for each instance $i$, we define the \textit{instance difference} $^{s_{1}}_{s_{2}}\Delta\acc_{i}$ as the difference in accuracy, i.e.
\begin{equation}
    ^{s_{1}}_{s_{2}}\Delta\acc_{i}  
    := \acc^{s_{2}}_{i}- \acc^{s_{1}}_{i}.
\end{equation}

To estimate this quantity from data, we first estimate instance accuracy $\acc^{s}_{i}$ from the data by averaging across 50 finetuning runs, and then take their differences to estimate the true difference.
We denote our estimate as $\hat{\acc}^{s}_{i}$ and $^{s_{1}}_{s_{2}}\hat{\Delta\acc}_{i}$.

As model size increases from $s_{1}$ to $s_{2}$, how are instance differences distributed?
Do all instances improve by a similar amount?
Or do they follow a Bernoulli-like distribution of ``either improving to totally correct, or ``not improving at all"?
Are there instances where bigger models are worse?
If so, how many? What are their properties?
Section \ref{sec:distr} answers the first three questions, Section \ref{sec:degrade} answers the fourth and the fifth, and Section \ref{sec:understanddegrade} answers the last.

\subsection{Distribution of Instance Difference} \label{sec:distr}
How is $^{s_{1}}_{s_{2}}\Delta\acc_{i}$ distributed, for example, when $s_{1}$ = \basesize and $s_{2}$ = \largesize?
To visualize this distribution, we first group instances that have similar estimated accuracy of the $\basesize$ model ($\hat{\acc}^{\basesize}$), and then for each group we plot the histogram of the estimated difference ($^{\basesize}_{\largesize}\hat{\Delta\acc}$). 
For example, we 1) select the group of instances $i$ where the \basesize model predicts correctly less than 5 out of 50 times, 2) for each instance in this group, we calculate how much more often \largesize model predicts correctly than \basesize , and 3) use a histogram to visualize how the difference is distributed across each instance.

Unfortunately, the estimation is always imperfect, and we want the observed properties of the estimated difference to hold for the true difference, instead of being an artifact of noisy estimation (\textit{false discoveries}).
Therefore, we introduce random ``mixing" baseline estimators $\overline{\acc}$ and $^{s_{1}}_{s_{2}}\overline{\Delta\acc}$ to control false discoveries. 
Whenever we compare smaller sizes ($s_{1}$) against bigger ($s_{2}$) ones, $\overline{\acc}^{s_{1}}$ estimates the accuracy by mixing predictions from 5 smaller pretrained models and 5 bigger ones (See Figure \ref{fig:mixing-estimator} for a more detailed illustration. ).
$\overline{\acc}^{s_{2}}$ estimates from the other 5 smaller and bigger models, and $^{s_{1}}_{s_{2}}\overline{\Delta\acc}$ is the difference between these two accuracy estimates. 
Intuitively, $^{s_{1}}_{s_{2}}\overline{\Delta\acc}$ has expectation 0 and captures only the noise aspect of $^{s_{1}}_{s_{2}}\hat{\Delta\acc}$.
When the true difference is 0, $\overline{\Delta\acc}$ and $\hat{\Delta\acc}$ are identical.
As a control, we plot the same histogram with the baseline estimators $\overline{\acc}$ and $\overline{\Delta\acc}$.

The resulting histograms are shown in Figure \ref{fig:improvement-hist}.
Compared to their baseline (blue), the estimated differences $^{\basesize}_{\largesize}\hat{\Delta\acc}$ (red):
\begin{itemize}
    \item are more widely spread (blue). 
    Hence, improvements from bigger models are not uniform across instances.
    \item have a longer tail on the left side of Figure \ref{fig:improvement-hist} (j). Hence, there are instances where bigger models predicts worse. 
    \item follow a unimodal distribution with smaller probability density further away from the mode.
    Hence, extreme values of instance difference are relatively rare (e.g. $\hat{\acc}$ rarely improves suddenly from 0 to 1).
\end{itemize}

We similarly plot $^{\minisize}_{\largesize}\hat{\Delta\acc}$ in Figure \ref{fig:improvement-hist-mini-large}.
When model size difference is larger, $\Delta\acc$ tend to be more extreme.
Particularly, there are more ``\textit{decay}" instances where the bigger model is worse.

\begin{figure*}%
    \centering
    \subfloat[\centering]{{\includegraphics[width=3cm]{Instance-level/figs/instance_diff-mnli-train_base-large-00.png} }}%
    \space
    \subfloat[\centering]{{\includegraphics[width=3cm]{Instance-level/figs/instance_diff-mnli-train_base-large-01.png} }}%
    \space
    \subfloat[\centering]{{\includegraphics[width=3cm]{Instance-level/figs/instance_diff-mnli-train_base-large-02.png} }}%
    \space
    \subfloat[\centering]{{\includegraphics[width=3cm]{Instance-level/figs/instance_diff-mnli-train_base-large-03.png} }}%
    \space
    \subfloat[\centering]{{\includegraphics[width=3cm]{Instance-level/figs/instance_diff-mnli-train_base-large-04.png} }}%
    \quad
    \subfloat[\centering]{{\includegraphics[width=3cm]{Instance-level/figs/instance_diff-mnli-train_base-large-05.png} }}%
    \space
    \subfloat[\centering]{{\includegraphics[width=3cm]{Instance-level/figs/instance_diff-mnli-train_base-large-06.png} }}%
    \space
    \subfloat[\centering]{{\includegraphics[width=3cm]{Instance-level/figs/instance_diff-mnli-train_base-large-07.png} }}%
    \space
    \subfloat[\centering]{{\includegraphics[width=3cm]{Instance-level/figs/instance_diff-mnli-train_base-large-08.png} }}%
    \space
    \subfloat[\centering]{{\includegraphics[width=3cm]{Instance-level/figs/instance_diff-mnli-train_base-large-09.png} }}%
    \caption{Comparing \basesize and \largesize at instance level. We estimate the instance accuracy $\hat{\acc}^{s}_{i}$ for each instance $i$ and model size $s=$ \basesize and $\largesize$, group them into different bins by their value of $\hat{\acc}^{\basesize}_{i}$, and use histogram to visualize the distribution of estimated instance difference $^{\basesize}_{\largesize}\hat{\Delta\acc}_{i}$ in red. 
    The blue bins represent the distribution of random baseline estimator $^{\basesize}_{\largesize}\overline{\Delta\acc}_{i}$.
    }%
    \label{fig:improvement-hist}%
\end{figure*}

\begin{figure}[h]%
    \centering
    \subfloat[\centering]{{\includegraphics[width=3cm]{Instance-level/figs/instance_diff-mnli-train_mini-large-00.png} }}%
    \space
    \subfloat[\centering]{{\includegraphics[width=3cm]{Instance-level/figs/instance_diff-mnli-train_mini-large-05.png} }}%
    \caption{Comparing \minisize and \largesize at instance level. We plot instance groups with $\hat{\acc}_{i}^{\minisize} \in [0, 0.1)$ (counterpart of Figure \ref{fig:improvement-hist} (a)) and $ \hat{\acc}^{\minisize}_{i} \in [0.5, 0.6)$ (counterpart of Figure \ref{fig:improvement-hist} (f)). 
    }%
    \label{fig:improvement-hist-mini-large}%
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{Instance-level/figs/mixingestimator.pdf}
    \caption{An illustration of the standard accuracy estimator $\hat{\acc}$ (above) and the ``random mixing baseline" $\overline{\acc}$ (below), which mixes a random half of smaller pretrained models and bigger ones.}
    \label{fig:mixing-estimator}
\end{figure}

\subsection{Decay Fraction for Bigger Models}\label{sec:degrade}
We have discovered a decay fraction (Figure \ref{fig:improvement-hist} red) of instances, and this fraction exceeds the false discovery control given by a baseline estimator (blue). 
However, this control seems heuristical. 
Is there any formal guarantees?
The answer is yes. Formally, we define the $\decay(t)$ as the fraction of instances $i$ where the estimated difference is smaller than a threshold $t$, i.e.

\begin{equation}
    \decay (t) := \mathbb{E}_{i}[\hat{\Delta\acc}_{i} < t],
\end{equation}

Correspondingly, the decay fraction given by the random baseline estimator is
\begin{equation}
    \overline{\decay} (t)  := \mathbb{E}_{i}[\overline{\Delta\acc}_{i} < t].
\end{equation}

We prove in Appendix \ref{sec:our-fdr-estimate} that if the bigger model is more accurate on every single instance,
then $\mathbb{E}[\overline{\decay} (t)] \geq \mathbb{E}[\decay (t)]$.
Therefore, $\overline{\decay}$ is indeed a baseline control with formal guarantees. 

Alternatively, we can follow a more traditional approach and use statistical significance to control false discoveries:
under the null hypothesis that bigger model is more accurate, what is the maximum probability $\alpha$ of the event $\hat{\Delta\acc}_{i} < t$?
Since both accuracy estimates $\hat{\acc}^{s_{1}}_{i}$ and $\hat{\acc}^{s_{2}}_{i}$ are binomial random variables, $\alpha$ can be easily computed. 

In fact, the previous statement lied a bit: $\hat{\acc}_{i}$ is not binomial; since some finetuning runs share the same pretraining seeds, the 50 finetuning runs are not entirely independent.
To make the traditional approach work and compare it against our method, we ensemble all 5 models with different finetuning seeds for each pretraining seeds. 
Hence we obtain 10 independent set of model predictions, and now $\hat{\acc}_{i}$ are binomial.

\begin{table}[]
    \centering
    \begin{tabular}{cccc}
    \hline
    Threshold & $\decay$ & $\overline{\decay}$ & $\alpha$ \\
    \hline
    $t = $\phantom{0}4 & 4.22E-2 &  3.49E-3 &   5.77E-2 \\
    $t = $\phantom{0}5 & 3.36E-2 &  6.90E-4 &   2.07E-2 \\
    $t = $\phantom{0}6 & 2.66E-2 &  1.22E-4 &   5.91E-3 \\
    $t = $\phantom{0}7 & 1.98E-2 &  1.73E-5 &   1.29E-3 \\
    $t = $\phantom{0}8 & 1.44E-2 &  1.80E-6 &   2.01E-4 \\
    $t = $\phantom{0}9 & 9.08E-3 &  1.44E-7 &   2.00E-5 \\
    $t = $10 & 4.75E-3 & 2.06E-8 &   9.54E-7   \\
    \hline
    \end{tabular}
    \caption{We compare \minisize vs. \largesize on MNLI in-domain development set, calculating how many fraction of instances $i$ have $\hat{\Delta\acc}_{i} \leq t$, along with the controls for false discoveries $\overline{\decay}$ and $\alpha$.}
    \label{tab:minivs.large}
\end{table}

We calculate the decay fraction $\decay(t)$ where \largesize is worse than \minisize in Table \ref{tab:minivs.large}, along with two false discovery controls $\overline{\decay}$ and $\alpha$. 
We find that
\begin{itemize}
    \item For $t \geq 5$, $\decay$ exceeds both controls. Hence, there are indeed instances where bigger models are worse.
    \item $\alpha$ is typically an order of magnitude larger than $\overline{\decay}$ and hence more conservative.
\end{itemize}

Taking the maximum difference of $\decay$ and $\overline{\decay}$ across $t$, we estimate $\minisize$ to be better than $\largesize$ on at least $2\%$ of the instances.


\subsection{Understanding the decay Fraction} \label{sec:understanddegrade}
What are the properties of the decay fraction of instances?
One hypothesis is that there are in fact no decay fraction: smaller model seems better at some instances only because they are wrongly annotated; if we correct them, will bigger models be be better on all instances?

To investigate this hypothesis, we manually examined the group of instances where $^{\minisize}_{\largesize}\hat{\Delta\acc}_{i} \geq 9$:
\minisize is almost always correct on these instances, while \largesize is almost always wrong. 
For each instance in this group, we manually categorize it into one of the four categories: 1) Correct, if the label is correct, 2) Fine, if the label might be controversial but we could see a reason why this label is reasonable, 3) Wrong, if the label is wrong, and 4) Unsure, if we are unsure how to label this instance.
As a control, we also examined the remaining fraction of the dataset.
Each time we annotate an instance, with $50\%$ probability it is sampled  from the decay fraction or the remaining fraction, and we do not know which group it comes from. 

The first author annotated 100 instances (degrade + control group) for each of the following three evaluation sets: MNLI in-domain development set, QQP in-domain development set, and SST-2.
Table \ref{tab:manual} shows the percentage of the four categories for both the decay fraction and the control group. 
\footnote{The second author follows the same procedure and reproduced the same qualitative results.}
Across all tasks:

\begin{itemize} 
    \item the decay fraction has higher percentage of noisy or wrong labels, compared to the remaining instances.
    \item after we adjust for the fraction of non-correct labels, the $\decay$ fraction in Table \ref{tab:minivs.large} still exceeds false discovery controls. 
    This implies that \minisize are better than \largesize on some correctly labeled instances.
\end{itemize}

However, we could not find an interpretable pattern for these decay fractions that are correctly labeled by simply eyeballing. 
We need additional information for each instance (e.g. meta-labels in Section \ref{sec:conclusion}) to gain more insights. 

\begin{table}[]
    \centering
    \begin{tabular}{rcccc}
     & Correct & Fine & Wrong & Unsure  \\
     \hline
   MNLI$^{D}$ & 66\% & 17\% & \phantom{0}9\% & \phantom{0}5\% \\
   MNLI$^{C}$ & 86\% & \phantom{0}5\% & 5\% & \phantom{0}1\% \\
   \hline
   SST-2$^{D}$ & 55\% & 8\% & 10\% & 25\%\\
   SST-2$^{C}$ & 88\% & \phantom{0}4\% & \phantom{0}0\% & \phantom{0}6\% \\
   \hline
   QQP$^{D}$  & 60\% & 26\% & 10\% & \phantom{0}2\% \\
   QQP$^{C}$  & 87\% & 10\% & \phantom{0}1\% & \phantom{0}0\% \\
   \hline
\end{tabular}
    \caption{We manually examine whether there are mislabels for instances where \minisize are better than \largesize (superscript $^D$), and the rest of the dataset (control group $^C$). }
    \label{tab:manual}
\end{table}
\fi









==> Instance-level/improvement_hist_old.tex <==
\section{Instance Difference} \label{sec:main-comparison-2models}
Since model predictions vary across random seeds, we cannot claim that certain model size $s$ predicts an instance $i$ completely (in)correctly.
Instead, we define the \textit{instance accuracy} $\acc^{s}_{i} \in [0, 1]$:
\begin{equation}
    \acc_{i}^{s} := \mathbb{E}_{P,F}[c^{i,s}].
\end{equation}
i.e. how often model of size $s$ predicts instance $i$ correctly.
When we compare two model sizes $s_{1}$ and $s_{2}$, for each instance $i$, we define the \textit{instance difference} $^{s_{1}}_{s_{2}}\Delta\acc_{i}$ as the difference in accuracy, i.e.
\begin{equation}
    ^{s_{1}}_{s_{2}}\Delta\acc_{i}  
    := \acc^{s_{2}}_{i}- \acc^{s_{1}}_{i}.
\end{equation}

As model size increases from $s_{1}$ to $s_{2}$, how are instance differences distributed?
Do all instances improve by a similar amount?
Or do they follow a Bernoulli-like distribution of ``either improving to totally correct, or ``not improving at all"?
Are there instances where bigger models are worse?
If so, how many? What are their properties?
Section \ref{sec:distr} answers the first three questions, Section \ref{sec:degrade} answers the fourth and the fifth, and Section \ref{sec:understanddegrade} answers the last.

\subsection{Estimating Instance Difference} \label{sec:diff-estimator}
We start by describing how to estimate instance differences $^{s_{1}}_{s_{2}}\Delta\acc_{i}$.
The true difference is not directly observable, so we first estimate instance accuracy $\acc^{s}_{i}$ from the data by averaging across 50 finetuning runs, and then take their differences to estimate the true difference.
We denote our estimate as $\hat{\acc}^{s}_{i}$ and $^{s_{1}}_{s_{2}}\hat{\Delta\acc}_{i}$.

Unfortunately, the estimation is always imperfect, and we want the observed properties of the estimated difference to hold for the true difference, instead of being an artifact of noisy estimation (\textit{false discoveries}).
Therefore, we introduce random ``mixing" baseline estimators $\underline{\acc}$ and $^{s_{1}}_{s_{2}}\underline{\Delta\acc}$ to control false discoveries. 
Whenever we compare smaller sizes ($s_{1}$) against bigger ($s_{2}$) ones, $\underline{\acc}^{s_{1}}$ estimates the accuracy by mixing predictions from 5 smaller pretrained models and 5 bigger ones.
$\underline{\acc}^{s_{2}}$ estimates from the other 5 smaller and bigger models, and $^{s_{1}}_{s_{2}}\underline{\Delta\acc}$ is the difference between these two accuracy estimates. 
Intuitively, $^{s_{1}}_{s_{2}}\underline{\Delta\acc}$ has expectation 0 and captures only the noise aspect of $^{s_{1}}_{s_{2}}\hat{\Delta\acc}$.
When the true difference is 0, $\underline{\Delta\acc}$ and $\hat{\Delta\acc}$ are identical.

\subsection{Distribution of Instance Difference} \label{sec:distr}
How is $^{s_{1}}_{s_{2}}\Delta\acc_{i}$ distributed, for example, when $s_{1}$ = \basesize and $s_{2}$ = \largesize?
To visualize this distribution, we first group instances that have similar estimated accuracy of the $\basesize$ model ($\hat{\acc}^{\basesize}$), and then for each group we plot the histogram of the estimated difference ($^{\basesize}_{\largesize}\hat{\Delta\acc}$). 
For example, we 1) select the group of instances $i$ where the \basesize model predicts correctly less than 5 out of 50 times, 2) for each instance in this group, we calculate how much more often \largesize model predicts correctly than \basesize , and 3) use a histogram to visualize how the difference is distributed across each instance.
To control false discoveries, we repeat the same procedure with the baseline estimators $\underline{\acc}$ and $\underline{\Delta\acc}$.

The resulting histograms are shown in Figure \ref{fig:improvement-hist}.
Compared to their baseline (blue), the estimated differences $^{\basesize}_{\largesize}\hat{\Delta\acc}$ (red)
\begin{itemize}
    \item are more widely spread than its baseline (blue). 
    Hence, improvements from bigger models are not uniform across instances.
    \item have a longer tail than  to the left side of Figure \ref{fig:improvement-hist} (j). Hence, there are instances where bigger models predicts worse. 
    \item follow a unimodal distribution with smaller probability density further away from the mode.
    Hence, extreme values of instance difference are relatively rare (e.g. $\hat{\acc}$ rarely improves suddenly from 0 to 1).
\end{itemize}

We similarly plot $^{\minisize}_{\largesize}\hat{\Delta\acc}$ in Figure \ref{fig:improvement-hist-mini-large}.
When model size difference is larger, $\Delta\acc$ tend to be more extreme.
Particularly, there are more ``\textit{degrading}" instances where the bigger model is worse.

\begin{figure*}%
    \centering
    \subfloat[\centering]{{\includegraphics[width=3cm]{Instance-resolution/figs/instance_diff-mnli-train_base-large-00.png} }}%
    \space
    \subfloat[\centering]{{\includegraphics[width=3cm]{Instance-resolution/figs/instance_diff-mnli-train_base-large-01.png} }}%
    \space
    \subfloat[\centering]{{\includegraphics[width=3cm]{Instance-resolution/figs/instance_diff-mnli-train_base-large-02.png} }}%
    \space
    \subfloat[\centering]{{\includegraphics[width=3cm]{Instance-resolution/figs/instance_diff-mnli-train_base-large-03.png} }}%
    \space
    \subfloat[\centering]{{\includegraphics[width=3cm]{Instance-resolution/figs/instance_diff-mnli-train_base-large-04.png} }}%
    \quad
    \subfloat[\centering]{{\includegraphics[width=3cm]{Instance-resolution/figs/instance_diff-mnli-train_base-large-05.png} }}%
    \space
    \subfloat[\centering]{{\includegraphics[width=3cm]{Instance-resolution/figs/instance_diff-mnli-train_base-large-06.png} }}%
    \space
    \subfloat[\centering]{{\includegraphics[width=3cm]{Instance-resolution/figs/instance_diff-mnli-train_base-large-07.png} }}%
    \space
    \subfloat[\centering]{{\includegraphics[width=3cm]{Instance-resolution/figs/instance_diff-mnli-train_base-large-08.png} }}%
    \space
    \subfloat[\centering]{{\includegraphics[width=3cm]{Instance-resolution/figs/instance_diff-mnli-train_base-large-09.png} }}%
    \caption{Comparing \basesize and \largesize at instance resolution. We estimate the instance accuracy $\hat{\acc}^{s}_{i}$ for each instance $i$ and model size $s=$ \basesize and $\largesize$, group them into different bins by their value of $\hat{\acc}^{\basesize}_{i}$, and use histogram to visualize the distribution of estimated instance difference $^{\basesize}_{\largesize}\hat{\Delta\acc}_{i}$ in red. 
    The blue bins represent the distribution of random baseline estimator $^{\basesize}_{\largesize}\underline{\Delta\acc}_{i}$.
    }%
    \label{fig:improvement-hist}%
\end{figure*}

\begin{figure}%
    \centering
    \subfloat[\centering]{{\includegraphics[width=3cm]{Instance-resolution/figs/instance_diff-mnli-train_mini-large-00.png} }}%
    \space
    \subfloat[\centering]{{\includegraphics[width=3cm]{Instance-resolution/figs/instance_diff-mnli-train_mini-large-05.png} }}%
    \caption{Comparing \minisize and \largesize at instance resolution. We plot instance groups with $\hat{\acc}_{i}^{\minisize} \in [0, 0.1)$ (counterpart of Figure \ref{fig:improvement-hist} (a)) and $ \hat{\acc}^{\minisize}_{i} \in [0.5, 0.6)$ (counterpart of Figure \ref{fig:improvement-hist} (f)). 
    }%
    \label{fig:improvement-hist-mini-large}%
\end{figure}

\subsection{Degrading Fraction for Bigger Models}\label{sec:degrade}
We have discovered a degrading fraction (Figure \ref{fig:improvement-hist} red) of instances, and this fraction exceeds the false discovery control given by a baseline estimator (blue). 
However, this control seems heuristical. 
Is there any formal guarantees?
The answer is yes. Formally, we define the $\degrade(t)$ as the fraction of instances $i$ where the estimated difference is smaller than a threshold $t$, i.e.

\begin{equation}
    \degrade (t) := \mathbb{E}_{i}[\hat{\Delta\acc}_{i} < t],
\end{equation}

Correspondingly, the degrading fraction given by the random baseline estimator is
\begin{equation}
    \underline{\degrade} (t)  := \mathbb{E}_{i}[\underline{\Delta\acc}_{i} < t].
\end{equation}

We prove in Appendix \ref{sec:our-fdr-estimate} that if the bigger model is more accurate on every single instance,
then $\mathbb{E}[\underline{\degrade} (t)] \geq \mathbb{E}[\degrade (t)]$.
Therefore, $\underline{\degrade}$ is indeed a reasonable baseline control with formal guarantees. 

Alternatively, we can follow a more traditional approach and use statistical significance to control false discoveries:
under the null hypothesis that bigger model is more accurate, what is the maximum probability $\alpha$ of the event $\hat{\Delta\acc}_{i} < t$?
Since both accuracy estimates $\hat{\acc}^{s_{1}}_{i}$ and $\hat{\acc}^{s_{2}}_{i}$ are binomial random variables, $\alpha$ can be easily computed. 

In fact, the previous sentence lied a bit: $\hat{\acc}_{i}$ is not binomial; since some finetuning runs share the same pretraining seeds, so the 50 finetuning runs are not entirely independent.
To make the traditional approach work and compare it against our method, we ensemble all 5 models with different finetuning seeds for each pretraining seeds. 
Hence we obtain 10 independent set of model predictions, and now $\hat{\acc}_{i}$ are binomial.

\begin{table}[]
    \centering
    \begin{tabular}{cccc}
    \hline
    Threshold & $\degrade$ & $\underline{\degrade}$ & $\alpha$ \\
    \hline
    $t = $\phantom{0}3 & 5.40E-2 &  3.12E-2 &   1.32E-1 \\
    $t = $\phantom{0}4 & 4.22E-2 &  1.36E-2 &   5.77E-2 \\
    $t = $\phantom{0}5 & 3.36E-2 &  3.89E-3 &   2.07E-2 \\
    $t = $\phantom{0}6 & 2.66E-2 &  1.29E-3 &   5.91E-3 \\
    $t = $\phantom{0}7 & 1.98E-2 &  1.67E-4 &   1.29E-3 \\
    $t = $\phantom{0}8 & 1.44E-2 &  1.85E-5 &   2.01E-4 \\
    $t = $\phantom{0}9 & 9.08E-3 &  9.70E-7 &   2.00E-5 \\
    $t = $10 & 4.75E-3 &  4.13E-8 &   9.54E-7   \\
    \hline
    \end{tabular}
    \caption{We compare \minisize vs. \largesize on MNLI in-domain development set, calculating how many fraction of instances $i$ have $\hat{d}^{i} \leq t$, along with its estimated false discovery rate $\fdr$.}
    \label{tab:minivs.large}
\end{table}

We calculate the degrading fraction $\degrade(t)$ where \largesize is worse than \minisize in Table \ref{tab:minivs.large}, along with two false discovery controls $\underline{\degrade}$ and $\alpha$. 
We find that
\begin{itemize}
    \item For $t \geq 5$, $\degrade$ exceeds both controls. Hence, there are indeed instances where bigger models are worse.
    \item $\alpha$ is typically an order of magnitude larger than $\underline{\degrade}$ and hence more conservative.
\end{itemize}

Taking the maximum difference of $\degrade$ and $\underline{\degrade}$ across $t$, we estimate $\minisize$ to be better than $\largesize$ on at least $2\%$ of the instances.


\subsection{Understanding the Degrading Fraction} \label{sec:understanddegrade}
What are the properties of the degrading fraction of instances?
One hypothesis is that there are in fact no degrading fraction: smaller model seems better at some instances only because they are wrongly annotated; if we correct them, will bigger models be be better on all instances?

To investigate this hypothesis, we manually examined the instances where $^{\minisize}_{\largesize}\hat{\Delta\acc}_{i} \geq 9$. 
For each instance, we categorize it into one of the four instance: 1) Correct, if the label is correct, 2) Fine, if the label might be controversial but we could see a reason why this label is reasonable, 3) Wrong, if the label is wrong, and 4) Unsure, if we are unsure how to label this instance.
As a control, we also examined the remaining fraction of the dataset.
Each time we annotate an instance, with $50\%$ probability it is sampled  from the degrading fraction or the remaining fraction, and we do not know which group it comes from. 

The first author annotated 100 instances (degrade + control group) for each of the following three evaluation sets: MNLI in-domain development set, QQP in-domain development set, and SST-2.
The results for both the degrading fraction and the control group can be seen in Table \ref{tab:manual}. 
\footnote{The second author follows the same procedure and reproduced the same qualitative results.}
We find that 

\begin{itemize} 
    \item Across all tasks, the degrading fraction has higher percentage of noisy or wrong labels, compared to the remaining instances.
    \item After we adjust for the fraction of correct labels, the $\degrade$ fraction in Table \ref{tab:minivs.large} still exceeds false discovery controls. 
    This implies that \minisize are better than \largesize on some correctly labeled instances.
\end{itemize}

However, we could not find an interpretable pattern for these degrading fractions that are correctly labeled by simply eyeballing. 
We need more additional information for each instance (e.g. meta-labels discussed in Section \ref{sec:conclusion}) to obtain more insights. 

\begin{table}[]
    \centering
    \begin{tabular}{rcccc}
     & Correct & Fine & Wrong & Unsure  \\
     \hline
   MNLI$^{D}$ & 66\% & 17\% & \phantom{0}9\% & \phantom{0}5\% \\
   MNLI$^{C}$ & 86\% & \phantom{0}5\% & 5\% & \phantom{0}1\% \\
   \hline
   SST-2$^{D}$ & 55\% & 8\% & 10\% & 25\%\\
   SST-2$^{C}$ & 88\% & \phantom{0}4\% & \phantom{0}0\% & \phantom{0}6\% \\
   \hline
   QQP$^{D}$  & 60\% & 26\% & 10\% & \phantom{0}2\% \\
   QQP$^{C}$  & 87\% & 10\% & \phantom{0}1\% & \phantom{0}0\% \\
   \hline
\end{tabular}
    \caption{We manually examine whether there are mislabels for instances where \minisize are better than \largesize (superscript $^D$), and the rest of the dataset (control group $^C$). }
    \label{tab:manual}
\end{table}









